Effects of Different Closure Choices in Core-Collapse Supernova Simulations

The two-moment method is widely used to approximate the full neutrino transport equation in core-collapse supernova (CCSN) simulations, and different closures lead to subtle differences in the simulation results. In this paper, we compare the effects of closure choices on various physical quantities in 1D and 2D time-dependent CCSN simulations with our multi-group radiation hydrodynamics code Fornax. We find that choices of the 3rd-order closure relations influence the time-dependent simulations only slightly. Choices of the 2nd-order closure relation have larger consequences than choices of the 3rd-order closure do, but these are still small compared to the remaining variations due to ambiguities in some physical inputs such as the nuclear equation of state. We also find that deviations in Eddington factors are not monotonically related to deviations in physical quantities, which means that simply comparing the Eddington factors does not inform one concerning which closure is better.

==> trash.tex <==
Neutrino mechanism has long been known to play an important role in the explosion of core collapse supernovae (CCSN). In ideal case, the 7-dimensional neutrino transport equation should be solved directly to reach high accuracy. Although some tests and simulations are done with this full Boltzmann neutrino transport \citep{smit2000,richers2017,nagakura2018,harada2019,harada2020,iwakami2020,iwakami2022}, the high computational cost of this method makes it almost impossible to be applied to a long-term, high spacial resolution, multi-dimensional (especially 3D) CCSN simulation today.

To reduce the computational cost, one widely used approach is the moment method. By taking the angular moments of the transport equation, the neutrino transport is now described by a series of moment equations, where the nth moment equation involves nth and (n+1)th angular moments. For non-static moving media, the (n+2)th angular moment is also present in the equation when a Lorentz transformation is applied between co-moving and lab frames \citep{just2015,skinner2019}. Therefore, to truncate at nth order and close the system, approximations of the (n+1)th moment (and in some cases the (n+2)th moment), the closure relations, are needed. In the simplest case, only 0th order equation which involves the energy density (0th moment), flux (1st moment) and pressure (2nd moment) is used, and this method is known as the diffusion approximation. Currently, the most commonly used method in CCSN simulations is to truncate at first order, also known as the M1 method \citep{murchikova2017} or the algebraic Eddington factor method \citep{just2015}, which requires the approximations of pressure (2nd moment) and heat (3rd moment) tensors. 

Various closures for the M1 method have been proposed in the literature (reference needed). The Wilson closure \citep{wilson1975} and Kershaw closure \citep{kershaw1976} were derived by interpolating the optically thin and thick limits. Since they were initially presented as flux limiters, they don't have corresponding closure for the 3rd moment. The Levermore closure \citep{levermore1984} is probably the most popular closure today. It assumes that there exists an inertial frame in which the radiation field is isotropic. Although Levermore's paper didn't mention 3rd moment, the corresponding closure for the 3rd moment can be found in \citep{vaytet2011}. Another set of widely used closures are the maximum entropy ones. The maximum entropy closures for Bose-Einstein radiation (MEBE), Fermi-Dirac radiation (MEFD) were proposed by \citep{cernohorsky1994}. Their classical limit was proposed earlier by \citep{minerbo1978}. The Levermore-Pomraning closure \citep{levermore1981} is the high occupation number limit of MEBE \citep{iwakami2022}, and thus it is not a suitable closure for neutrino distributions. Given 0th and 1st moments, these closures find the most likely angular distribution function by maximizing the entropy of the radiation field. The Janka closures were presented in \citep{janka1991,janka1992}. They were based on fitting to the Monte Carlo simulations in the proto-neutron star (PNS) envelope. The Nagakura closure was proposed in \citep{nagakura2021}, where the angular distribution of neutrinos is fitted from a spherical symmetric CCSN model with full Boltzmann transport.

To test the performance of these closures, two types of comparisons have been made. One is to compare with the Monte Carlo simulations \citep{janka1992,murchikova2017,richers2017} and the other is to compare to discrete-ordinate (SN) method \citep{smit2000,richers2017,nagakura2018,harada2019,harada2020,iwakami2020,iwakami2022}. In 1D, the Eddington factors extracted from simulations and closures are compared. These works commonly pointed out that at the early stage of a CCSN there are regions where Eddington factor is smaller than $1/3$ \citep{iwakami2022} but only Wilson and MEFD closures can give such situations. The latter is favored because it satisfies the causality requirement \cite{smit2000}. With multi-dimensional simulations, the stress tensor of the Eddington tensor are compared element-wise or by principal-axis analysis \citep{harada2019,iwakami2020,iwakami2022}. These comparisons show that the principal axis directions predicted by the closures can deviate from the simulations, and applying the closures in the lab frame or in the co-moving frame makes a difference as well. 

However, due to the high computation cost of the MC and SN methods, the multi-dimensional comparisons can only be done in a very short timescale or at several time slices. As a result, although investigations have shown that different choices of closures and simulation methods may make a difference in short period, we have little knowledge on how the CCSN will respond to such differences between closures and how much the physical quantities of an explosion are influenced \citep{mezzacappa2022}. Do these differences act just as if there are some random perturbations to the star, or they have systematic consequences?

